Context-Dependent Models for Predicting and Characterizing Facial Expressiveness

In recent years, extensive research has emerged in affective computing on topics like automatic emotion recognition and determining the signals that characterize individual emotions. Much less studied, however, is expressiveness, or the extent to which someone shows any feeling or emotion. Expressiveness is related to personality and mental health and plays a crucial role in social interaction. As such, the ability to automatically detect or predict expressiveness can facilitate significant advancements in areas ranging from psychiatric care to artificial social intelligence. Motivated by these potential applications, we present an extension of the BP4D+ dataset with human ratings of expressiveness and develop methods for (1) automatically predicting expressiveness from visual data and (2) defining relationships between interpretable visual signals and expressiveness. In addition, we study the emotional context in which expressiveness occurs and hypothesize that different sets of signals are indicative of expressiveness in different contexts (e.g., in response to surprise or in response to pain). Analysis of our statistical models confirms our hypothesis. Consequently, by looking at expressiveness separately in distinct emotional contexts, our predictive models show significant improvements over baselines and achieve comparable results to human performance in terms of correlation with the ground truth.

==> bayesian.tex <==
\begin{figure*}
    \centering
    \includegraphics{expressiveness/fig_mlm.pdf}
    \caption{Posterior density plots for each feature in each task. A blue plot indicates that a feature is associated with significantly more expressiveness and a red plot indicates that a feature is associated with significantly less expressiveness. Black dots indicate point estimates (posterior medians) and error bars represent interval estimates (highest density intervals).}
    \label{fig:mlm}
\end{figure*}

\begin{table*}[]
    \centering
    \begin{tabular}{l ccc c ccc c ccc}
        \toprule
         & \multicolumn{3}{c}{Startle Task} && \multicolumn{3}{c}{Pain Task} && \multicolumn{3}{c}{Disgust Task} \\
        \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
        Parameter & Est. & 95\% HDI & pd && Est. &
        95\% HDI & pd && Est. & 95\% HDI & pd \\
        \midrule
        Intercept       & --0.06 & [--0.13, 0.01] & 94.5\% &&
                          0.08 & [0.00, 0.15] & 97.7\% &&
                          0.04 & [--0.06, 0.14] & 81.0\% \\
        AU Count        & 0.10 & [0.04, 0.17] & 99.8\% &&
                          0.25 & [0.18, 0.32] & 100\% &&
                          0.40 & [0.33, 0.48] & 100\% \\
        Points Displ.   & 0.92 & [0.73, 1.13] & 100\% &&
                          0.15 & [--0.01, 0.32] & 96.2\% &&
                          0.86 & [0.62, 1.14] & 100\% \\
        Points Veloc.   & 0.30 & [0.21, 0.40] & 100\% &&
                          --0.16 & [--0.31, --0.03] & 98.9\% &&
                          0.18 & [0.01, 0.37] & 98.4\% \\
        Pitch Displ.    & 0.08 & [0.01, 0.15] & 98.1\% &&
                          --0.06 & [--0.18, 0.06] & 85.1\% &&
                          0.12 & [--0.01, 0.26] & 96.6\% \\
        Pitch Veloc.    & 0.04 & [--0.03, 0.11] & 84.2\% &&
                          0.20 & [0.08, 0.31] & 100\% &&
                          --0.05 & [--0.16, 0.05] & 82.9\% \\
        Yaw Displ.      & 0.00 & [--0.08, 0.09] & 50.2\% &&
                          0.05 & [--0.05, 0.16] & 84.7\% &&
                          0.13 & [--0.04, 0.29] & 94.2\% \\
        Yaw Veloc.      & --0.04 & [--0.13, 0.06] & 77.9\% &&
                          0.03 & [--0.08, 0.13] & 68.4\% &&
                          0.11 & [--0.02, 0.24] & 95.9\% \\
        \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}
